Optimality-Informed Neural Networks for Solving Parametric Optimization Problems

Many engineering tasks require solving families of nonlinear constrained optimization problems, parametrized in setting-specific variables. This is computationally demanding, particularly if solutions have to be computed across strongly varying parameter values, e.g., in real-time control or for model-based design. Thus, we propose to learn the mapping from parameters to the primal optimal solutions and to their corresponding duals using neural networks, giving a dense estimation in contrast to gridded approaches. Our approach, Optimality-Informed Neural Networks (OptINNs), combines (i) a KKT-residual loss that penalizes violations of the first-order optimality conditions under standard constraint qualification assumptions, and (ii) problem-specific output activations that enforce simple inequality constraints (e.g., box-type/positivity) by construction. This design reduces data requirements, allows the prediction of dual variables, and improves feasibility and closeness to optimality compared to penalty-only training. Taking quadratic penalties as a baseline, as previously proposed for this problem class in the literature, our method simplifies hyperparameter tuning and attains tighter adherence to optimality conditions. We evaluate OptINNs on different nonlinear optimization problems ranging from low to high dimensions and compare them with equally sized neural networks trained using the quadratic-penalty method. On small problems, OptINNs match a quadratic-penalty baseline in primal accuracy while additionally predicting dual variables with low error. On larger problems, OptINNs achieve lower constraint violations, lower primal error, and lower errors in the predicted costs. These results suggest that embedding feasibility and optimality into the network architecture and loss can make learning-based surrogates more accurate, feasible, and data-efficient for parametric optimization.

==> data/results/rocket_car/optinn/rocket_car_optinn_u_error_colormap.tex <==
% colour bar of rocket_car_optinn_u_error_colormap: error -0.254 … 0.254, bisymlog, linthresh=0.000254
\pgfplotsset{colormap={rocket_car-optinn-u}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-optinn-u/.style={
    colormap name=rocket_car-optinn-u,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.865297,-0.535276,-0.231121,0,0.231121,0.535276,0.865297}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.965443,-0.850088,-0.83309,-0.813828,-0.791603,-0.765335,-0.733219,-0.691883,-0.633801,-0.520423,-0.503871,-0.485178,-0.463708,-0.438489,-0.407929,-0.369141,-0.315994,-0.219092,-0.205972,-0.191544,-0.175516,-0.15749,-0.136895,-0.112876,0.112876,0.136895,0.15749,0.175516,0.191544,0.205972,0.219092,0.315994,0.369141,0.407929,0.438489,0.463708,0.485178,0.503871,0.520423,0.633801,0.691883,0.733219,0.765335,0.791603,0.813828,0.83309,0.850088,0.965443}}}}


==> data/results/rocket_car/optinn/rocket_car_optinn_v_error_colormap.tex <==
% colour bar of rocket_car_optinn_v_error_colormap: error -0.252 … 0.252, bisymlog, linthresh=0.000252
\pgfplotsset{colormap={rocket_car-optinn-v}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-optinn-v/.style={
    colormap name=rocket_car-optinn-v,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.866439,-0.536392,-0.232034,0,0.232034,0.536392,0.866439}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.966586,-0.851229,-0.834231,-0.814968,-0.792742,-0.766473,-0.734356,-0.693018,-0.634931,-0.521536,-0.50498,-0.486282,-0.464806,-0.439578,-0.409005,-0.370196,-0.31701,-0.219985,-0.206842,-0.192384,-0.176321,-0.15825,-0.137596,-0.113496,0.113496,0.137596,0.15825,0.176321,0.192384,0.206842,0.219985,0.31701,0.370196,0.409005,0.439578,0.464806,0.486282,0.50498,0.521536,0.634931,0.693018,0.734356,0.766473,0.792742,0.814968,0.834231,0.851229,0.966586}}}}


==> data/results/rocket_car/optinn/rocket_car_optinn_x_error_colormap.tex <==
% colour bar of rocket_car_optinn_x_error_colormap: error -0.289 … 0.289, bisymlog, linthresh=0.000289
\pgfplotsset{colormap={rocket_car-optinn-x}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-optinn-x/.style={
    colormap name=rocket_car-optinn-x,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.846663,-0.517084,-0.21642,0,0.21642,0.517084,0.846663}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.946783,-0.831459,-0.814468,-0.795215,-0.773002,-0.74675,-0.714659,-0.673365,-0.615365,-0.502284,-0.485798,-0.467189,-0.44583,-0.420764,-0.39043,-0.352004,-0.299539,-0.204732,-0.192016,-0.178074,-0.162644,-0.145372,-0.125756,-0.103058,0.103058,0.125756,0.145372,0.162644,0.178074,0.192016,0.204732,0.299539,0.352004,0.39043,0.420764,0.44583,0.467189,0.485798,0.502284,0.615365,0.673365,0.714659,0.74675,0.773002,0.795215,0.814468,0.831459,0.946783}}}}


==> data/results/rocket_car/qpnn/rocket_car_qpnn_u_error_colormap.tex <==
% colour bar of rocket_car_qpnn_u_error_colormap: error -0.254391 … 0.254391, bisymlog, linthresh=0.000254391
\pgfplotsset{colormap={rocket_car-qpnn-u}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-qpnn-u/.style={
    colormap name=rocket_car-qpnn-u,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.865076,-0.535059,-0.230944,0,0.230944,0.535059,0.865076}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.965221,-0.849866,-0.832869,-0.813606,-0.791381,-0.765114,-0.732998,-0.691662,-0.633581,-0.520207,-0.503655,-0.484963,-0.463494,-0.438277,-0.40772,-0.368936,-0.315797,-0.218919,-0.205804,-0.191381,-0.17536,-0.157342,-0.136759,-0.112755,0.112755,0.136759,0.157342,0.17536,0.191381,0.205804,0.218919,0.315797,0.368936,0.40772,0.438277,0.463494,0.484963,0.503655,0.520207,0.633581,0.691662,0.732998,0.765114,0.791381,0.813606,0.832869,0.849866,0.965221}}}}


==> data/results/rocket_car/qpnn/rocket_car_qpnn_v_error_colormap.tex <==
% colour bar of rocket_car_qpnn_v_error_colormap: error -0.251741 … 0.251741, bisymlog, linthresh=0.000251741
\pgfplotsset{colormap={rocket_car-qpnn-v}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-qpnn-v/.style={
    colormap name=rocket_car-qpnn-v,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.866587,-0.536537,-0.232153,0,0.232153,0.536537,0.866587}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.966734,-0.851377,-0.834379,-0.815116,-0.79289,-0.766621,-0.734504,-0.693165,-0.635077,-0.521681,-0.505124,-0.486426,-0.464948,-0.439719,-0.409145,-0.370334,-0.317142,-0.220102,-0.206955,-0.192494,-0.176426,-0.158348,-0.137687,-0.113577,0.113577,0.137687,0.158348,0.176426,0.192494,0.206955,0.220102,0.317142,0.370334,0.409145,0.439719,0.464948,0.486426,0.505124,0.521681,0.635077,0.693165,0.734504,0.766621,0.79289,0.815116,0.834379,0.851377,0.966734}}}}


==> data/results/rocket_car/qpnn/rocket_car_qpnn_x_error_colormap.tex <==
% colour bar of rocket_car_qpnn_x_error_colormap: error -0.288792 … 0.288792, bisymlog, linthresh=0.000288792
\pgfplotsset{colormap={rocket_car-qpnn-x}{
    rgb=(0.0196,0.1882,0.3804)
    rgb=(0.0368,0.2215,0.4265)
    rgb=(0.0541,0.2547,0.4727)
    rgb=(0.0713,0.2879,0.5188)
    rgb=(0.0885,0.3211,0.5649)
    rgb=(0.1057,0.3543,0.6111)
    rgb=(0.1230,0.3875,0.6572)
    rgb=(0.1425,0.4173,0.6834)
    rgb=(0.1634,0.4450,0.6975)
    rgb=(0.1843,0.4727,0.7116)
    rgb=(0.2052,0.5003,0.7258)
    rgb=(0.2261,0.5280,0.7399)
    rgb=(0.2471,0.5557,0.7541)
    rgb=(0.2749,0.5842,0.7689)
    rgb=(0.3235,0.6149,0.7855)
    rgb=(0.3721,0.6457,0.8021)
    rgb=(0.4328,0.6841,0.8228)
    rgb=(0.4814,0.7149,0.8394)
    rgb=(0.5300,0.7456,0.8561)
    rgb=(0.5774,0.7750,0.8720)
    rgb=(0.6161,0.7947,0.8830)
    rgb=(0.6549,0.8144,0.8941)
    rgb=(0.6937,0.8341,0.9052)
    rgb=(0.7324,0.8537,0.9163)
    rgb=(0.7712,0.8734,0.9273)
    rgb=(0.8099,0.8931,0.9384)
    rgb=(0.8371,0.9063,0.9444)
    rgb=(0.8605,0.9174,0.9487)
    rgb=(0.8839,0.9285,0.9530)
    rgb=(0.9073,0.9396,0.9573)
    rgb=(0.9306,0.9506,0.9616)
    rgb=(0.9540,0.9617,0.9659)
    rgb=(0.9709,0.9579,0.9502)
    rgb=(0.9746,0.9406,0.9206)
    rgb=(0.9783,0.9234,0.8911)
    rgb=(0.9820,0.9062,0.8616)
    rgb=(0.9857,0.8890,0.8321)
    rgb=(0.9894,0.8717,0.8025)
    rgb=(0.9908,0.8505,0.7698)
    rgb=(0.9852,0.8173,0.7273)
    rgb=(0.9797,0.7841,0.6849)
    rgb=(0.9742,0.7509,0.6424)
    rgb=(0.9686,0.7176,0.6000)
    rgb=(0.9631,0.6844,0.5576)
    rgb=(0.9576,0.6512,0.5151)
    rgb=(0.9407,0.6099,0.4813)
    rgb=(0.9223,0.5675,0.4487)
    rgb=(0.9038,0.5250,0.4161)
    rgb=(0.8807,0.4720,0.3753)
    rgb=(0.8623,0.4295,0.3427)
    rgb=(0.8438,0.3871,0.3101)
    rgb=(0.8226,0.3433,0.2863)
    rgb=(0.8005,0.2990,0.2654)
    rgb=(0.7783,0.2547,0.2444)
    rgb=(0.7562,0.2104,0.2235)
    rgb=(0.7340,0.1661,0.2026)
    rgb=(0.7119,0.1218,0.1817)
    rgb=(0.6807,0.0886,0.1659)
    rgb=(0.6346,0.0738,0.1585)
    rgb=(0.5885,0.0591,0.1511)
    rgb=(0.5423,0.0443,0.1437)
    rgb=(0.4962,0.0295,0.1363)
    rgb=(0.4501,0.0148,0.1290)
    rgb=(0.4039,0.0000,0.1216)
},
  rocket_car-qpnn-x/.style={
    colormap name=rocket_car-qpnn-x,
    point meta min=-1,
    point meta max=1,
    colorbar style={ytick={-0.846767,-0.517185,-0.216501,0,0.216501,0.517185,0.846767}, yticklabels={$-10^{-1}$,$-10^{-2}$,$-10^{-3}$,$0$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, minor ytick={-0.946887,-0.831563,-0.814572,-0.795319,-0.773105,-0.746854,-0.714763,-0.673468,-0.615468,-0.502386,-0.485899,-0.467289,-0.44593,-0.420863,-0.390527,-0.3521,-0.299631,-0.204811,-0.192092,-0.178148,-0.162715,-0.145438,-0.125816,-0.103111,0.103111,0.125816,0.145438,0.162715,0.178148,0.192092,0.204811,0.299631,0.3521,0.390527,0.420863,0.44593,0.467289,0.485899,0.502386,0.615468,0.673468,0.714763,0.746854,0.773105,0.795319,0.814572,0.831563,0.946887}}}}

